Learning diffusion at lightspeed

Diffusion regulates numerous natural processes and the dynamics of many successful generative models. Existing models to learn the diffusion terms from observational data rely on complex bilevel optimization problems and model only the drift of the system. We propose a new simple model, JKOnet*, which bypasses the complexity of existing architectures while presenting significantly enhanced representational capabilities: JKOnet* recovers the potential, interaction, and internal energy components of the underlying diffusion process. JKOnet* minimizes a simple quadratic loss and outperforms other baselines in terms of sample efficiency, computational complexity, and accuracy. Additionally, JKOnet* provides a closed-form optimal solution for linearly parametrized functionals, and, when applied to predict the evolution of cellular processes from real-world data, it achieves state-of-the-art accuracy at a fraction of the computational cost of all existing methods. Our methodology is based on the interpretation of diffusion processes as energy-minimizing trajectories in the probability space via the so-called JKO scheme, which we study via its first-order optimality conditions.

==> chapters/_old_parametrizations.tex <==
\section{Training}
\label{sec:algorithms}

Let us recall the learning objective: Given a sequence of sample populations $(\mu_0,\mu_1,\ldots,\mu_T)$, where each population $\mu_t=\frac{1}{N}\sum_{i=1}^N\delta_{x_i}$ consists of finitely many samples $x_i\in\reals^d$ of the population, we seek to infer the energy functional $J$ that generated them.
% In all settings proposed so far, we considered the energy function to belong to some general class of functionals (e.g., potential energy with continuously differentiable and lower bounded potential, energy functional with unknown parameters, etc.). 
In this section, we consider the case of parametrized by a finite set of parameters $\theta\in\reals^n$ and study the case of linear function approximation (\cref{subsec:linear_approximation}) and nonlinear function approximation (\cref{subsec:neural_network}).

\subsection{Linear Function Approximation}\label{subsec:linear_approximation}

Suppose the energy functional at absolutely continuous measures $\d\mu=\rho(x)\d x$ can be parametrized as
\begin{equation}\label{eq:linear_approximation:energy}
\begin{aligned}
    J_{\theta}(\mu)
    &=
    \int_{\reals^d}\theta_1^\top \phi_1(x)\d\mu(x)
    \\
    &+
    \int_{\reals^d}\theta_2^\top \phi_2(x-y)\d(\mu\times\mu)(x,y)
    \\
    &+
    \theta_3\int_{\reals^d}\rho(x)\log(\rho(x))\d x,
\end{aligned}
\end{equation}
where $\theta=(\theta_1^\top,\theta_2^\top,\theta_3)^\top\in\reals^{2n+1}$, $\theta_1, \theta_2\in\reals^n$, $\theta_3\in\nonnegativeReals$, and $\phi_1,\phi_2:\reals^n\to\reals^n$ are sufficiently well-behaved.
% \begin{remark}
% Two remarks are in order. First, we assume with no loss of generality that $\theta_1$ and $\theta_2$ have the same dimension. Second, if $\theta_3$ is dropped, the entropy term disappears and the objective remains well-defined even at measures that are not absolutely continuous.  
% \end{remark}
% We now show the learning problem (i.e., the optimization problem~\eqref{eq:general:learning_objective}) admits a closed-form solution for the parameters of the energy functional~\eqref{eq:linear_approximation:energy}: 
The minimization of \eqref{eq:general:learning_objective} admits a closed-form solution:
\begin{proposition}\label{prop:linear_approximation}
    Assume that the features $\phi_{1,i}$ and $\phi_{2,i}$ are continuously differentiable, bounded, and have bounded Hessian. Define the matrix $y:\reals^d\to\reals^{(2n+1)\times d}$ by 
    \begin{equation*}
        y(x_t)
        \!\coloneqq\!
        \left(\gradient\phi(x_{t})^\top, \int_{\reals^d}\gradient\phi(x_{t}\!-\!x_{t}')^\top\d\mu_t(x_t'), \frac{\gradient\rho(x_t)}{\rho(x_t)}\right)^\top
    \end{equation*}
    and suppose that the data is sufficiently exciting so that %the matrix 
    \begin{equation}\label{eq:linear_approximation:potential:invertible}
        \sum_{t=1}^{T}
        \int_{\reals^d}
        y_t(x_t)y_t(x_t)^\top\d\mu_t(x_t).
    \end{equation}
    is invertible.
    Then, the optimal solution of~\eqref{eq:general:learning_objective} reads
    \begin{equation}\label{eq:linear_approximation:optimal}
    \begin{aligned}
        \theta^\ast
        &=
        \frac{1}{\tau}
        \left(
            \sum_{t=1}^{T} \int_{\reals^d}y(x_t)y(x_t)^\top\d\mu_t(x_t)
        \right)^{-1}
        \\
        &\quad
        \left(
            \sum_{t=0}^{T-1}\int_{\reals^d\times\reals^d} y(x_{t+1})(x_{t+1}-x_t)\d\gamma_t(x_t,x_{t+1})
        \right).
    \end{aligned}
    \end{equation}
\end{proposition}

\subsection{Nonlinear Function Approximation}\label{subsec:neural_network}

We now turn our attention to nonlinear function approximations. As above, we express the energy functional at absolutely continuous measures $\d\mu=\rho(x)\d x$, but we now use neural networks for the potential and the interaction energies: 
\begin{align*}
    J_{\theta}(\mu)
    &=
    \int_{\reals^d}V_{\theta_1}(x)\d\mu(x)
    \\
    &+
    \int_{\reals^d}U_{\theta_2}(x-y)\d(\mu\times\mu)(x,y)
    \\
    &+
    \theta_3\int_{\reals^d}\rho(x)\log(\rho(x))\d x,
\end{align*}
where $V_{\theta_1}:\reals^d\to\reals$ and $U_{\theta_2}:\reals^d\to\reals$ are neural networks parametrized by $\theta_1$ and $\theta_2$, respectively\footnote{Boundedness and differentiability are the only neural network's requirements.}.
As in~\cref{subsec:linear_approximation}, our methodology simply consists of minimizing the loss~\eqref{eq:general:learning_objective}. Since there is now no closed-form solution, we use gradient descent on the parameters $\theta$. 

\begin{remark}
    As above, the computation of the optimal couplings $\gamma_t\in\setPlans{\mu_t}{\mu_{t+1}}$ and, if $\theta_3$ is not set to zero, the estimation the densities $\rho_t$ of $\mu_t$ and their gradient $\gradient{}\rho_t$ can be perform offline before the learning task; cf. \cref{fig:system}.
\end{remark}

\subsection{Details}
% \paragraph{Discussion}
A few comments are in order. 
% \emph{Special cases.}
% By ``dropping'' the corresponding term in $J_\theta$,~\cref{prop:linear_approximation} readily extends to the case with an arbitrary combination of the energies. For instance, in the case of potential energy only, we obtain the optimal solution 
% \begin{multline*}
%     \theta_1^\ast
%     =
%     \frac{1}{\tau}
%     \left(
%         \sum_{t=1}^{T}\int_{\reals^d}\gradient\phi_1(x_{t})\gradient\phi_1(x_{t})^\top\d\mu_t(x_t)
%     \right)^{-1}
%     \\
%     \left(
%         \sum_{t=0}^{T-1}\int_{\reals^d\times\reals^d}\gradient\phi_1(x_{t+1})(x_{t+1}-x_t))\d\gamma_t(x_t,x_{t+1})
%     \right).
% \end{multline*}

\emph{Computation of the optimal couplings.}
\textcolor{red}{TODO}

\emph{Estimation of $\rho$ and $\gradient\rho$.}
The case with $\theta_3$ non-zero imposes to compute and estimate of the density $\rho_t$ and its gradient $\gradient\rho_t$ given the empirical probability measures $\mu_t$. For instance, these estimated quantities can be estimated via a mixture of Gaussians. Other approaches are based on normalizing flows, \ldots. This complexity, instead, is bypassed if there no internal energy. 

\emph{Regularization.}
Of course, one might additionally regularize the optimization problem by penalizing the norm $\theta$. 
% or the norm of the potential function $V_{\theta_1}$ in the space $\Lp{2}{\reals^d;\reals;\mu_t}$, the norm of the interaction function $U_{\theta_2}$ in the space $\Lp{2}{\reals^d\times\reals^d;\reals;\mu_t\times\mu_t}$, and $\beta_3^2$ at each time $t$ (each weighted by some non-negative constant).
% Since all regularization terms are quadratic (e.g., $\norm{V_\theta}_{\Lp{2}{\reals^d,\reals;\mu_t}}^2=\int_{\reals^d}\theta_1^\top\phi_1(x)\phi_1(x)^\top \theta_1\d\mu_t(x)$), a closed-form solution continues to exist $\theta$.
Just like in standard least squares, regularization can be used, among others, to alleviate bad conditioning of the matrix~\eqref{eq:linear_approximation:potential:invertible}. 

% \emph{Nonnegativity of $\theta_3$.}
% Strictly speaking, the parameter $\theta_3$ resulting from~\eqref{eq:linear_approximation:optimal} cannot be guaranteed to ensure the non-negativity constraint. Non-negativity must therefore be checked a posteriori and/or can be enforced using regularization techniques.

% \newpage 





% Three options:
% \begin{enumerate}
% \item Synthetic datasets, and keep applications for follow up work (real-world application, without cutting corners)
%     \begin{enumerate}
%     \item Improve on Charlotte 
%     \item Generate trajectories (via different functionals) and learn them
%     \item one with density fitting
% \end{enumerate}
% \item Real-world application but cutting corner (else remove focus from methodological contribution)
% \item Both
% \end{enumerate}

==> utils/tikzart.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{shapes}

\RequirePackage{tikz}
\usetikzlibrary{decorations.pathreplacing,shapes.misc,pgfplots.fillbetween}

\definecolor{ETHblue}{RGB}{33,92,175}% blue
\definecolor{ETHpetrol}{RGB}{0,120,148}	% petrol
\definecolor{ETHgreen}{RGB}{98,115,19}% green
\definecolor{ETHbronze}{RGB}{142,103,19}% bronze
\definecolor{ETHred}{RGB}{183,53,45}% red
\definecolor{ETHpurple}{RGB}{163,7,116}	% purple
\definecolor{ETHgray}{RGB}{111,111,111}% gray

\tikzset{remblais/.style={circle, fill=ETHred, inner sep=0pt,minimum size=7pt}}
\tikzset{deblais/.style={fill=ETHblue,minimum size=3pt}}
\tikzset{variation/.style={draw=ETHbronze,-latex,thick}}

%OT
\newcommand{\transportMapContinuous}[2]{
    % raw material
\draw (0,0) -- (4,0);
\draw[fill=gray!25] (0.25,0) to [curve through={(.5,-0.1) . . (1,-0.75) . . (1.5,-0.5) . . (2,-.45) . . (2.75,-1) . . (3.5,-0.25)}] (3.75,0) -- cycle;
\node (nu) at (2,.25) {\ifstrempty{#1}{$\mu$}{#1}};

% construction
\draw (5,0) -- (8,0);
\draw[fill=gray!25] (5.25,0) -- (5.25,1.5) -- (5.75,1.5) -- (5.75,1) -- (6.5,1) -- (6.5,2) -- (7.25,1.5) -- (7.75,1.5) -- (7.75,0) -- cycle;
\node (nu) at (7,-.3) {\ifstrempty{#2}{$\nu$}{#2}};

% transport map
\draw[draw=blue, thick, -latex] (3,-.25) to [bend left] node[midway,above left] {$T(x)$} (6,.5);
}
\newcommand{\transportMapDiscrete}{
    % sources
    \node[deblais] (s1) at (0,0) {};
    \node[deblais] (s2) at (3,2) {};
    \node[deblais] (s3) at (2,-1) {};
    \node[deblais] (s4) at (3,.5) {};
    
    % destinatinons
    \node[remblais] (d1) at (0,2) {};
    \node[remblais] (d2) at (1,1) {};
    \node[remblais] (d3) at (4,0) {};
    
    % transport map
    \draw[draw=blue,-latex] (s1) to (d1);
    \draw[draw=blue,-latex] (s2) to (d2);
    \draw[draw=blue,-latex] (s3) to (d2);
    \draw[draw=blue,-latex] (s4) to (d3);
}

\newcommand{\transportPlanContinuous}[3]{
    % box
    \coordinate (bl) at (2,0);
    \coordinate (tl) at ($(bl) + (0,4)$);
    \draw (bl) -- ($(bl) + (4,0)$) -- ($(bl) + (4,4)$) -- (tl) -- cycle;
    
    % raw material
     \draw[fill=gray!25] ($(bl) + (0,0.25)$) to [curve through={($(bl) + (-0.1,.5)$) . . ($(bl) + (-0.75,1)$) . . ($(bl) + (-0.5,1.5)$) . . ($(bl) + (-.45,2)$) . . ($(bl) + (-1,2.75)$) . . ($(bl) + (-0.25,3.5)$)}] ($(bl) + (0,3.75)$) -- cycle;
    \node[anchor=east] (mu) at ($(bl) + (-.5,1.8)$) {\ifstrempty{#1}{$\mu$}{#1}};
     
    % construction
    \coordinate (shifttl) at ($(tl) + (1,0)$);
    \draw[fill=gray!25] ($(shifttl) + (0.25,0)$) -- ($(shifttl) + (0.25,1.5)$) -- ($(shifttl) + (0.75,1.5)$) -- ($(shifttl) + (0.75,1)$) -- ($(shifttl) + (1.5,1)$) -- ($(shifttl) + (1.5,2)$) -- ($(shifttl) + (2.25,1.5)$) -- ($(shifttl) + (2.75,1.5)$) -- ($(shifttl) + (2.75,0)$) -- cycle;
    \node (nu) at ($(tl) + (2.5,.5)$) {\ifstrempty{#2}{$\nu$}{#2}};
    
    % transport plan
    % TODO make precise... right now marginal make no sense
    \path[draw,use Hobby shortcut,closed=true,fill=blue!25] (4.25,0.5) .. (5,1) .. (5.5,.5) .. (5.5,2) .. (5.5,3) .. (5,3) .. (4,3.25) .. (4,2.5);
    
    \node (gamma) at ($(bl) + (3,2)$) {\ifstrempty{#3}{$\plan{\gamma}$}{#3}};
}

\newcommand{\transportPlanDiscrete}{
    % sources
    \node[deblais] (s1) at (0,0) {};
    \node[deblais] (s2) at (3,2) {};
    \node[deblais] (s3) at (2,-1) {};
    \node[deblais] (s4) at (3,.5) {};
    
    % destinatinons
    \node[remblais] (d1) at (0,2) {};
    \node[remblais] (d2) at (1,1) {};
    \node[remblais] (d3) at (4,0) {};
    
    % transport map
    \draw[draw=blue,-latex] (s1) to (d1);
    \draw[draw=blue,-latex] (s1) to (d2);
    \draw[draw=blue,-latex] (s2) to (d1);
    \draw[draw=blue,-latex] (s2) to (d2);
    \draw[draw=blue,-latex] (s3) to (d2);
    \draw[draw=blue,-latex] (s4) to (d3);
}

\newcommand{\geodesicsOriginalSpace}{
    \node[deblais] (x) at (0,0) {};
    \node[remblais] (y) at (2,0) {};
    
    % \draw[dashed] (x) to[bend left=90] (y);
    \draw[dashed] (x) -- (y);
    \draw[dashed] (x) to[bend right=90] (y);
    \draw[blue, -latex] plot [smooth] coordinates {(x.south) (0.5,-.5) (1.5,.5) (y.north)};
}
\newcommand{\geodesicsProbabilitySpaceDiscrete}[1]{
    \node[deblais] (x1) at (0,0) {};
    \node[remblais] (y1) at (2,0) {};
    \node[deblais] (x2) at (0,2) {};
    \node[remblais] (y2) at (2,2) {};
\ifstrempty{#1}{
    \draw[dashed] (x2) to[bend left] (y1);
    \draw[dashed] (x1) -- (y2);
    
    \draw[blue,-latex] plot [smooth] coordinates {(x1.south) (0.5,-.5) (1.5,.5) (y1.north)};;
    \draw[blue,-latex] (x2) -- (y2);
}{
    \draw[dashed] (x2) -- (y2);
    \draw[dashed] plot [smooth] coordinates {(x1.south) (0.5,-.5) (1.5,.5) (y1.north)};
    \draw[red,-latex] (x2) to[bend left] (y1);
    \draw[red,-latex] (x1) -- (y2);
}
}

\newcommand{\geodesicsProbabilitySpaceContinuous}[2]{
    \draw[dashed, thick] (1,-.25) to [bend left=90] (7,.75);
    \draw[dashed, thick] (2,-.25) to [bend right=90] (7,.5);
    
    \transportMapContinuous{#1}{#2}
}

%SPP
% Code adapted from https://tex.stackexchange.com/questions/57668/drawing-a-flag-with-tikz
\newcommand{\destination}[3]{%
\begin{scope}[scale=#2,rotate=#3]
    \draw[fill=brown!60!black,thick] ($#1 + (0,0)$) -- ++ (0,8) arc (180:0:0.4 and 0.1) -- ++ (0,-8) arc (360:180:0.4 and 0.1);
    \draw[thick] ($#1 + (0,8)$) arc (180:360:0.4 and 0.1);
    \draw[fill=blue,thick] ($#1 + (0.8,7.5)$) to[out=-30,in=210] ++(3,0) to[out=30,in=150] ++ (3,0) -- ++ (0,-3) to [out=150,in=30] ++(-3,0) to[out=210,in=-30] ++(-3,0) -- cycle;
\end{scope}
}

\tikzset{
 pics/obstacle/.style={
   code={
   \draw[use Hobby shortcut, draw=black, fill, closed] (0,0) +($(0:1+4*rnd)$)
       \foreach \a in {60,120,...,350} {  .. +($(\a: 1+4*rnd)$) };
   }
}}

% https://github.com/sisl/aircraftshapes
\pgfdeclareshape{quadcopter top}{
\inheritsavedanchors[from=coordinate]
\inheritanchor[from=coordinate]{center}
\backgroundpath{
\begin{pgfscope}
\pgftransformshift{\centerpoint}
\pgfmathdivide{\pgfkeysvalueof{/pgf/minimum width}}{1pt}
\pgftransformscale{\pgfmathresult}
\pgfpathcircle{\pgfpoint{0}{0}}{0.08}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.24}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.24}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.24}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.24}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.21}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.21}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.21}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.21}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.25}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.25}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.25}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.25}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.025}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.025}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.025}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.025}
\pgfpathmoveto{\pgfpoint{-0.01}{0}}
\pgfpathlineto{\pgfpoint{0.25}{0.26}}
\pgfpathlineto{\pgfpoint{0.27}{0.26}}
\pgfpathlineto{\pgfpoint{0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{0.01}{0}}
\pgfpathlineto{\pgfpoint{-0.25}{0.26}}
\pgfpathlineto{\pgfpoint{-0.27}{0.26}}
\pgfpathlineto{\pgfpoint{-0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{-0.01}{0}}
\pgfpathlineto{\pgfpoint{0.25}{-0.26}}
\pgfpathlineto{\pgfpoint{0.27}{-0.26}}
\pgfpathlineto{\pgfpoint{0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{0.01}{0}}
\pgfpathlineto{\pgfpoint{-0.25}{-0.26}}
\pgfpathlineto{\pgfpoint{-0.27}{-0.26}}
\pgfpathlineto{\pgfpoint{-0.01}{0}}
\pgfpathclose
\end{pgfscope}}}

% Forest ride
\newcommand{\forestRideFlag}[1]{
    \destination{(row#1) + (flags)}{0.04}{22.5};
}
\newcommand{\forestRideAgent}[3]{
    \node [quadcopter top,fill=white,draw=#3,minimum width=0.4cm,rotate=360*rnd] at ($(col#2) + (row#1)$) {};
}
\newcommand{\drawForestRideWorld}{
    \draw[step=.5,black,thin] (-0.25,-0.25) grid (12.75,5.25);
    % YOU SHALL NOT PASS LINE
    \draw[draw=red, thick] (0, -0.25) -- (0,5.25);
    
    % define columns and rows
    \foreach \col in {0,...,24}
        \coordinate (col\col) at (0.25 + 0.5*\col,0);
    \foreach \row in {0,...,9}
        \coordinate (row\row) at (0,4.75 - 0.5*\row);
        
    % TREES
    \foreach \row/\col in {0/11,0/12,0/13,0/14,0/15,0/20,2/13,2/14,4/16,4/17,6/11,6/12,6/13,6/14,8/17,8/18,9/15,9/16,9/17} {
        \pic at ($(col\col) + (row\row)$)  [fill=black!60!green, scale=0.06, rotate=360*rnd]{obstacle};
     }
     
     \coordinate (flags) at ($(col24) + (-0.1,-0.2)$);
}

\newcommand{\IFAheart}{
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and (-1.5,1.00) .. (-1.5,2)  arc (180:0:0.75);
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and ( 1.5,1.00) .. ( 1.5,2)  arc (0:180:0.75);
\node[inner sep=0pt] (ifa) at (0,1.5)
    {\includegraphics[width=.2\textwidth]{utils/logos/ifalogo_color.pdf}};
}

\newcommand{\subgradients}{
% \begin{axis}[width=1.2\textwidth]
\draw[very thin, dashed, color=gray, step=2] (0.0,0.0) grid (12,10);
\draw [very thick,  domain=0:2, samples=5, smooth, variable=\t]
    plot ({\t}, {-2*\t + 8});
\draw [very thick,  domain=2:4, samples=5, smooth, variable=\t]
    plot ({\t}, {\t*\t*0.25 + 3});
\draw [very thick,  domain=4:8, samples=10, smooth, variable=\t]
    plot ({\t}, {(\t-8)*(\t-8)*5*0.0625 + 2});
\draw [very thick,  domain=8:9, samples=5, smooth, variable=\t]
    plot ({\t}, {2});
\draw [very thick,  domain=9:12, samples=5, smooth, variable=\t]
    plot ({\t}, {9});
\draw[dashed, very thick] (9,2) -- (9,9);
\node[mark size=2pt,color=black] at (9,2) {\pgfuseplotmark{*}};
\node[mark size=2pt,color=black] at (9,9) {\pgfuseplotmark{o}};
% \end{axis}
}
